Identification of emotions on Twitter during the 2022 electoral process in Colombia

The study of Twitter as a means for analyzing social phenomena has gained interest in recent years due to the availability of large amounts of data in a relatively spontaneous environment. Within opinion-mining tasks, emotion detection is specially relevant, as it allows for the identification of people's subjective responses to different social events in a more granular way than traditional sentiment analysis based on polarity. In the particular case of political events, the analysis of emotions in social networks can provide valuable information on the perception of candidates, proposals, and other important aspects of the public debate. In spite of this importance, there are few studies on emotion detection in Spanish and, to the best of our knowledge, few resources are public for opinion mining in Colombian Spanish, highlighting the need for generating resources addressing the specific cultural characteristics of this variety. In this work, we present a small corpus of tweets in Spanish related to the 2022 Colombian presidential elections, manually labeled with emotions using a fine-grained taxonomy. We perform classification experiments using supervised state-of-the-art models (BERT models) and compare them with GPT-3.5 in few-shot learning settings. We make our dataset and code publicly available for research purposes.

==> tables/cantidad_por_etiquetador.tex <==
\begin{table}
\centering
\scriptsize
\begin{tabular}{lrrr}
\toprule
Emocion & Cantidad etiquetador 1 & Cantidad etiquetador 2 & Cantidad etiquetador 3 \\
\midrule
Alegria & 61 & 107 & 125 \\
Agrado & 2 & 36 & 59 \\
Confianza & 417 & 242 & 395 \\
Admiración & 79 & 25 & 292 \\
Miedo & 84 & 98 & 76 \\
Incertidumbre & 37 & 28 & 74 \\
Sorpresa & 6 & 3 & 4 \\
Asombro & 1 & 15 & 5 \\
Tristeza & 18 & 10 & 57 \\
Decepción & 137 & 119 & 74 \\
Asco & 82 & 119 & 374 \\
Desagrado & 494 & 357 & 463 \\
Ira & 26 & 111 & 161 \\
Odio & 23 & 0 & 115 \\
Otra & 4 & 11 & 21 \\
Neutro & 107 & 111 & 115 \\
\bottomrule
\end{tabular}
\caption{Cantidad de tweets asignados a cada emocion por etiquetador}
\label{table:tweets_etiquetador}
\end{table}


==> tables/emotions_table.tex <==
\begin{longtable}{{ | l | p{13cm} |}}
\caption{Descripción de las emociones usadas} \label{table:emotions_description} \\
\toprule
Emoción & Descripción \\
\midrule
\endfirsthead
\caption[]{Descripción de las emociones usadas} \\
\toprule
Emoción & Descripción \\
\midrule
\endhead
\midrule
\multicolumn{2}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
Admiración & La admiración es una emoción social que se siente al observar a personas de competencia, talento o habilidad que superan los estándares. La admiración facilita el aprendizaje social en grupos. La admiración motiva la superación personal a través del aprendizaje de los modelos a seguir. \\
Agrado & Sensación moderada de felicidad o placer que siente una persona por algo que le gusta. \\
Confianza & La confianza implica que una parte se vuelve vulnerable ante otra, asumiendo que esta actuará en su beneficio.En una relación de confianza, el que confía no controla las acciones del otro. \\
Alegría & Es una emoción positiva que suele ir acompañada de bienestar. Se genera como resultado de un evento positivo. \\
Incertidumbre & La incertidumbre es la falta de seguridad, de confianza o de certeza sobre algo. Aparece en situaciones en las que no tenemos control total, en las que nos faltan respuestas e información, y nos puede generar inquietud, inseguridad, estrés, ansiedad e incluso miedo \\
Miedo & El miedo surge ante amenazas reales o imaginarias de daño físico, emocional o psicológico. En textos, se muestra como amenazas hacia el autor del mensaje o lo que se menciona, cuando está vulnerable o en desventaja.  \\
Asombro & La condición de estar asombrado; un estado de asombro abrumador, como por sorpresa o miedo repentino, horror o admiración.  \\
Sorpresa & Se define como una reacción provocada por algo inesperado, extraño o novedoso para la persona. En el texto está principalmente asociada a resultados inesperados o descubrimientos singulares respecto al enunciado del tweet. \\
Decepción & La decepción es la insatisfacción que sigue al fracaso de expectativas o esperanzas. A diferencia del arrepentimiento que se centra en elecciones personales, la decepción se enfoca en el resultado en sí. Puede generar estrés psicológico. \\
Tristeza & La tristeza es un dolor emocional causado por decadencia espiritual, manifestándose en llanto, abatimiento, falta de apetito, cansancio, etc. Ocurre cuando las expectativas no se cumplen o las circunstancias son dolorosas.  \\
Desagrado & Una actitud o un sentimiento de disgusto o aversión. \\
Asco & Contiene una serie de estados con intensidades variables que van desde una leve aprensión hasta una intensa repulsión. Todos los estados de asco se desencadenan por la sensación de que algo es aversivo, repulsivo y/o tóxico.  \\
Odio & El odio es una intensa respuesta emocional negativa hacia ciertas personas, cosas o ideas, generalmente relacionadas con la oposición o repulsión hacia algo. El odio a menudo se asocia con intensos sentimientos de ira, desprecio y disgusto. \\
Ira & La ira surge por objetivos no alcanzados o trato injusto, pudiendo ser peligrosa y relacionada con la violencia. En el texto, el autor reta o reclama por un derecho vulnerado, buscando justicia. \\
\end{longtable}


==> tables/errorrs_2.2.tex <==
\begin{table}[t]
\scriptsize
\centering
\begin{tabularx}{\textwidth}{|>{\raggedright\arraybackslash}X|>{\raggedright\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\raggedright\arraybackslash}X|}
\hline
\textbf{Text} & \textbf{Labels} & \textbf{Preds GPT} & \textbf{Reasoning} & \textbf{Interpretation} \\
\hline
"@petrogustavo Petro por favor no te desgastes mas con ese patan, mejor haz el reclamo en la registraduria, se sabe que ganamos en primera vuelta!!!" & Alegría & "Alegría, Asco" & El autor manifiesta su confianza en la victoria de Petro y menciona que el reclamo debería hacerse en la Registraduría. Además, califica negativamente al oponente como 'patán'. La respuesta final es: Alegría, Asco. & Capta la componente de alegría y detecta solamente con una palabra "patán" el desagrado con uno de los candidatos. \\
\hline
"@FicoGutierrez Colombia te dijo QUE NO! vaya a llorar y deje la lamboneria a ver si le dan un cargo publico.. en el futuro gobierno de los corruptos de Hernandez, si llega... le daria algun cargo al patetico este? ""Embajador en Cuba""" & Asco & "Asco, Miedo" & El autor se expresa de manera despectiva ("llorar", "lamboneria") hacia el posible gobierno de Hernández y hacia Petro. Además, expresa su aversión hacia el futuro incierto. La respuesta final es: Asco, Miedo. & Aquí hay un error claro en la apreciación de miedo. Sobreinterpreta la oración en términos del miedo al futuro. \\
\hline
"yo diria; viejo loco demente y corrupto, contra hombre honesto, luchador y con la mente mas brillante del panorama politico." & Asco & "Asco, Alegría" & El autor expresa su desprecio hacia el ex guerrillero y le atribuye adjetivos negativos como "loco" y "corrupto". Por otro lado, muestra su apoyo y admiración por el ingeniero, al cual describe como honesto y brillante. La respuesta final es: Asco, Alegría. & \\
\hline
\end{tabularx}
\caption{Type 2 errors examples}
\label{table:errors_2}
\end{table}

==> tables/errors_1.1.tex <==
\begin{table}[t]
    \captionsetup{font=scriptsize} % Set caption font size
    \footnotesize
    \centering
    \begin{tabularx}{\textwidth}{|>{\raggedright\arraybackslash}X|>{\raggedright\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\raggedright\arraybackslash}X|}
        \hline
        \textbf{Text}                                                                                                                                                                                                   & \textbf{Labels} & \textbf{Preds GPT 1} & \textbf{Chain of Thought 2}                                                                                                                                                                                                & \textbf{Interpretation 3}                                                                                         \\
        \hline
        Escuchar que cuando entrevistan a Petro, se aprende de Historia, de Macroeconomia, de Politicas Verdes y cuando entrevistan a Fico, estoy revisando si me robaron el celular, la billetera, da susto el tipo... & Alegría, Asco   & Alegría, Asco, Miedo & El autor expresa su apoyo y admiración por Petro, resaltando sus cualidades y conocimientos. Por otro lado, expresa desprecio y miedo hacia Fico, considerándolo una amenaza. La respuesta final es: Alegría, Asco, Miedo. & Capta bien la componente de apoyo a un candidato y desagrado al otro... no ve la ironía en el comentario del robo \\
        \hline
        @lcvelez @lafm una alternativa para ejercer el derecho a estar informados como electores, que no escondan al viejito, no les de pena. @petrogustavo ya está listo.                                              & Asco            & Alegría              & El autor expresa su apoyo hacia la idea de un debate obligatorio para ejercer el derecho a estar informados y critica la actitud de esconder al candidato mayor. La respuesta final es: Alegría.                           & No ve la ironía en el uso de términos como "viejito"                                                              \\
        \hline
        Desde muy temprano apoyando a Marbelle en su sueño de irse del país. relieved face relieved face                                                                                                                & Asco            & Alegría              & El autor expresa su apoyo y entusiasmo hacia Marbelle en su decisión de irse del país, lo cual refleja positividad y celebración. La respuesta final es: Alegría.                                                          & No ve la ironía en el hecho de apoyar la salida del país de una persona                                           \\
        \hline
        %@FernanMartinez Ya perdiste Fernan. Tiene 4 años para hacer oposición, disfrútalos. & Alegría & Tristeza, Asco & El autor muestra su desprecio y desánimo hacia Fernan al indicar que ya perdió, aconsejándole disfrutar los 4 años de oposición. La respuesta final es: Tristeza, Asco. & Es un comentario con evidente grado de ironía, en tanto se burla de la derrota. \\
        \hline
    \end{tabularx}
    \caption{Type 1 errors examples}
    \label{table:errors_1}
\end{table}

==> tables/errors_1.tex <==
\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{{ | p{1.5cm}| p{4.5cm} | p{1.8cm} | p{1.8cm} | p{3.5cm} |}}
\hline
\textbf{Text} & \textbf{Labels} & \textbf{Preds GPT 1} & \textbf{Chain of Thought 2} & \textbf{Interpretation 3} \\
\hline
Escuchar que cuando entrevistan a Petro ,se aprende de Historia,de Macroeconomia,de Politicas Verdes y cuando entrevistan a Fico ,estoy revisando si me robaron el celular,la billetera ,da susto el tipo... & Alegría,Asco & Alegría,Asco,Miedo & El autor expresa su apoyo y admiración por Petro, resaltando sus cualidades y conocimientos. Por otro lado, expresa desprecio y miedo hacia Fico, considerándolo una amenaza. La respuesta final es: Alegría, Asco, Miedo. & Capta bien la componente de apoyo a un candidato y desagrado al otro... no ve la ironía en el comentario del robo \\
\hline
@lcvelez @lafm una alternativa para ejercer el derecho a estar informados como electores, que no escondan al viejito, no les de pena. @petrogustavo ya esta listo. & Asco & Alegría & El autor expresa su apoyo hacia la idea de un debate obligatorio para ejercer el derecho a estar informados y critica la actitud de esconder al candidato mayor. La respuesta final es: Alegría. & No ve la ironía en el uso de términos como "viejito" \\
\hline
Desde muy temprano apoyando a Marbelle en su sueno de irse del pais. relieved face relieved face & Asco & Alegría & El autor expresa su apoyo y entusiasmo hacia Marbelle en su decisión de irse del país, lo cual refleja positividad y celebración. La respuesta final es: Alegría. & No ve la ironía en el hecho de apoyar la salida del país de una persona \\
\hline
@FernanMartinez Ya perdiste Fernan. Tiene 4 anos para hacer oposicion, disfrutalos. & Alegría & Tristeza,Asco & El autor muestra su desprecio y desánimo hacia Fernan al indicar que ya perdió, aconsejándole disfrutar los 4 años de oposición. La respuesta final es: Tristeza, Asco. & Es un con evidente grado de ironía, en tanto se burla de la derrota. \\
\hline
\end{tabular}
\caption{Type 1 errors examples}
\label{table:errors_1}
\end{table}

==> tables/errors_2.tex <==
\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{|p{1.5cm}|p{3cm}|p{1.5cm}|p{1.5cm}|p{4.5cm}|p{4.5cm}|}
\hline
Text & Labels & Preds GPT & Reasoning & Interpretation \\
\hline
"@petrogustavo Petro por favor no te desgastes mas con ese patan, mejor haz el reclamo en la registraduria, se sabe que ganamos en primera vuelta!!!" & Alegría & "Alegría,Asco" & El autor manifiesta su confianza en la victoria de Petro y menciona que el reclamo debería hacerse en la Registraduría. Además, califica negativamente al oponente como 'patán'. La respuesta final es: Alegría, Asco. & Capta la componente de alegría y detecta solamente con una palabra "patán" el desagrado con uno de los candidatos. \\
"@FicoGutierrez Colombia te dijo QUE NO! vaya a llorar y deje la lamboneria a ver si le dan un cargo publico.. en el futuro gobierno de los corruptos de Hernandez, si llega... le daria algun cargo al patetico este? "" Embajador en Cuba""" & Asco & "Asco,Miedo" & El autor se expresa de manera despectiva ("llorar", "lamboneria") hacia el posible gobierno de Hernández y hacia Petro. Además, expresa su aversión hacia el futuro incierto. La respuesta final es: Asco, Miedo. & Aquí hay un error claro en la apreciación de miedo. Sobreinterpreta la oración en términos del miedo al futuro. \\
"yo diria; viejo loco demente y corrupto, contra hombre honesto, luchador y con la mente mas brillante del panorama politico." & Asco & "Asco,Alegría" & El autor expresa su desprecio hacia el ex guerrillero y le atribuye adjetivos negativos como "loco" y "corrupto". Por otro lado, muestra su apoyo y admiración por el ingeniero, al cual describe como honesto y brillante. La respuesta final es: Asco, Alegría. & \\
\hline
\end{tabular}
\caption{Type 2 errors examples}
\label{table:errors_2}
\end{table}


==> tables/errors_21.1.tex <==
\begin{table}[t]
\scriptsize
\centering
\begin{tabularx}{\textwidth}{|>{\raggedright\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\raggedright\arraybackslash}X|>{\raggedright\arraybackslash}X|}
\hline
\textbf{Text} & \textbf{Labels} & \textbf{Preds GPT} & \textbf{Reasoning} & \textbf{Interpretation} \\
\hline
Pobres de nuestros niños y quedan en manos de los hermanos Benedetti el plan de Gustavo Petro es darle a la hermana de Armando @AngelaBenedet el control del ICBF @ultimahorapp @PublimetroCol @pulzo @Las2Orillas @zonacero & Asco & "Tristeza,Asco" & El texto expresa preocupación y desprecio por la situación de los niños al quedar en manos de los hermanos Benedetti, además muestra aversión hacia el plan de Gustavo Petro. La respuesta final es: Tristeza, Asco. & Claramente aquí palabras como "pobres de nuestros niños" son interpretadas de forma literal en su connotación de tristeza, cuando lo que están expresando es desagrado con la situación. \\
\hline
Como ya se sabe que va a ganar el Retrogrado Rodolfo Hernandez por orden de las grandes elites mafiosas de comombia, pues que tiemble las grandes elites mafiosas politiqueras de Colombia, pues él, Rodolfo, va a acabar con la CORRUPCION & Asco & "Alegría,Asco" & El autor expresa su confianza en la victoria de Rodolfo Hernández y su desprecio hacia las élites mafiosas, además muestra apoyo hacia la lucha contra la corrupción. La respuesta final es: Alegría, Asco. & No nota el uso irónico del texto general. \\
\hline
\end{tabularx}
\caption{Type 2.1 errors examples}
\label{table:errors_21}
\end{table}

==> tables/errors_21.tex <==
\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{|p{5cm}|p{3cm}|p{3cm}|p{5cm}|p{5cm}|}
\hline
Text & Labels & Preds GPT & Reasoning & Interpretation \\
\hline
Pobres de nuestros niños y quedan en manos de los hermanos Benedetti el plan de Gustavo Petro es darle a la hermana de Armando @AngelaBenedet el control del ICBF @ultimahorapp @PublimetroCol @pulzo @Las2Orillas @zonacero & Asco & "Tristeza,Asco" & El texto expresa preocupación y desprecio por la situación de los niños al quedar en manos de los hermanos Benedetti, además muestra aversión hacia el plan de Gustavo Petro. La respuesta final es: Tristeza, Asco. & Claramente aquí palabras como "pobres de nuestros hermanos" son interpretadas de forma literal en su connotación de tristeza, cuando lo que están expresando es desagrado con la situación. \\
Como ya se sabe que va a ganar el Retrogrado Rodolfo Hernandez por orden de las grandes elites mafiosas de comombia, pues que Tiemble las grandes elites mafiosas potiqueras de Colombia, pues el, Rodolfo, va a acabar con la CORRUPCION & Asco & "Alegría,Asco" & El autor expresa su confianza en la victoria de Petro y su desprecio hacia Rodolfo Hernández, a quien considera parte de las élites mafiosas. Además, muestra apoyo hacia la lucha contra la corrupción. La respuesta final es: Alegría, Asco. & No nota el uso irónico de general del texto \\
\hline
\end{tabular}
\caption{Type 2.1 errors examples}
\label{table:errors_21}

\end{table}


==> tables/errors_3.1.tex <==
\begin{table}[t]
    \tiny
    \centering
    \begin{tabularx}{\textwidth}{|>{\raggedright\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\raggedright\arraybackslash}X|>{\raggedright\arraybackslash}X|}
        \hline
        \textbf{Text}                                                                                                                                                              & \textbf{Labels} & \textbf{Preds GPT} & \textbf{Reasoning}                                                                                                                                                                                                & \textbf{Interpretation}                                                                                                       \\
        \hline
        !Que nervios! A 30 minutos que se vaya la luz en todo el pais, se apaguen las emisoras y amanezcamos con una contundente victoria de @FicoGutierrez                        & Alegría, Miedo  & Miedo              & El autor expresa su nerviosismo ante la incertidumbre de lo que pueda suceder en las elecciones, mostrando preocupación. La respuesta final es: Miedo.                                                            & Capta bien la componente de incertidumbre pero no logra visualizar la alegría, expresada en la idea de "contundente victoria" \\
        \hline
        Yo de @IvanDuque ya iria militarizado Colombia... y q nos vayan avisando si hay q buscar armas para defendernos a los civiles.                                             & Miedo, Asco     & Miedo              & El autor expresa su preocupación y temor ante la posibilidad de militarizar Colombia y la necesidad de armarse para defenderse, mostrando así sentimientos de inquietud y ansiedad. La respuesta final es: Miedo. & Capta la componente de incertidumbre                                                                                          \\
        \hline
        No es objetivo. Me parece que los moderadores estan parcializados. Esperaba un poco mas de @NoticiasCaracol pero bueno...Que mas se espera de un medio privado colombiano. & Tristeza, Asco  & Tristeza           & El autor expresa su descontento ante lo que considera un debate parcializado, mostrando su decepción y desconfianza hacia los moderadores y el medio privado colombiano. La respuesta final es: Tristeza.         & No llega a captar una componente vinculada al desagrado de la situación                                                       \\
        \hline
        @ElQueLosDELATA !Manana con toda en las urnas para derrotar a esta banda de mafiosos!                                                                                      & Alegría, Asco   & Alegría            & El autor expresa entusiasmo y apoyo hacia la jornada electoral del día siguiente, con el objetivo de derrotar a quienes considera como una banda de mafiosos. La respuesta final es: Alegría.                     & No llega a captar la componente de desagrado en "esta banda de mafiosos"                                                      \\
        \hline
    \end{tabularx}
    \caption{Type 3 errors examples}
    \label{table:errors_3}
\end{table}

==> tables/errors_3.tex <==
\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{|p{5cm}|p{3cm}|p{3cm}|p{5cm}|p{5cm}|}
\hline
Text & Labels & Preds GPT & Reasoning & Interpretation \\
\hline
!Que nervios! A 30 minutos que se vaya la luz en todo el pais, se apaguen las emisoras y amanezcamos con una contundente victoria de @FicoGutierrez & Alegría, Miedo & Miedo & El autor expresa su nerviosismo ante la incertidumbre de lo que pueda suceder en las elecciones, mostrando preocupación. La respuesta final es: Miedo. & Capta bien la componente de incertidumbre pero no logra visualizar la alegría, expresada en la idea de "contundente victoria" \\
Yo de @IvanDuque ya iria militarizado Colombia... y q nos vayan avisando si hay q buscar armas para defendernos a los civiles. & Miedo, Asco & Miedo & El autor expresa su preocupación y temor ante la posibilidad de militarizar Colombia y la necesidad de armarse para defenderse, mostrando así sentimientos de inquietud y ansiedad. La respuesta final es: Miedo. & Capta la componente de incertidumbre \\
No es objetivo. Me parece que los moderadores estan parcializados. Esperaba un poco mas de @NoticiasCaracol pero bueno...Que mas se espera de un medio privado colombiano. & Tristeza, Asco & Tristeza & El autor expresa su descontento ante lo que considera un debate parcializado, mostrando su decepción y desconfianza hacia los moderadores y el medio privado colombiano. La respuesta final es: Tristeza. & No llega a captar una componente vinculada al desagrado de la situación \\
@ElQueLosDELATA !Manana con toda en las urnas para derrotar a esta banda de mafiosos! & Alegría, Asco & Alegría & El autor expresa entusiasmo y apoyo hacia la jornada electoral del día siguiente, con el objetivo de derrotar a quienes considera como una banda de mafiosos. La respuesta final es: Alegría. & No llega a captar la componente de desagrado en "esta banda de mafiosos" \\
\hline
\end{tabular}
\caption{Type 3 errors examples}
\label{table:errors_3}
\end{table}


==> tables/labels.tex <==
\begin{table}
\caption{Tweets etiquetados}
\label{table:labeled_tweets}
\begin{tabular}{lllll}
\toprule
 & Alegria & Miedo & Tristeza & Asco \\
\midrule
Cantidad de tweets & 93 & 22 & 20 & 112 \\
Etiquetados correctamente & 81 & 9 & 15 & 97 \\
F1 score & 0.89 & 0.419 & 0.577 & 0.847 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/labels_counts.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{rr}
\toprule
Cantidad de etiquetas & Cantidad de Tweets \\
\midrule
0 & 123 \\
1 & 909 \\
2 & 165 \\
3 & 2 \\
\bottomrule
\end{tabular}
\caption{Cantidad de tweets por cantidad de etiquetas finales asignadas}
\label{table:labels_counts}
\end{table}


==> tables/models_descriptions.tex <==
\begin{table}[!htbp]
\scriptsize
\begin{tabular}{{ | l | p{13cm} |}}
\hline
Modelo & Descripcion  \\
\hline
robertuito  & Modelo de lenguaje preentrenado para contenido generado por usuarios en español, entrenado siguiendo las pautas de RoBERTa en 500 millones de tweets. \\
bertin & Modelo basados en RoBERTa entrenados desde cero en la parte española de mC4 usando Flax \\
electricidad & Modelo base tipo Electra entrenado en el corpus BETO \\
beto & BETO es un modelo BERT entrenado con un gran corpus español. \\
roberta & Modelo base de RoBERTa y ha sido preentrenado utilizando un corpus en español de 570 GB de texto limpio  \\
twitter-xlm & Modelo basado en XLM-roBERTa multilingüe entrenado en ~198 millones de tweets y ajustado para el análisis de sentimientos. \\
\hline
\end{tabular}
\caption{Descripción de los modelos usados}
\label{table:model_description}
\end{table}


==> tables/trendings_clean.tex <==

\begin{longtable}{lllr}
\caption{Hashtags} \label{table:hashtags} \\
\toprule
date & trending & Sector & Count \\
\midrule
\endfirsthead
\caption[]{Hashtags} \\
\toprule
date & trending & Sector & Count \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{Continua en la siguiente pagina} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
2022-05-22 & NosUnimosONosJodemos & Derecha & 427 \\
2022-05-22 & FedericoEsColombia & Derecha & 1597 \\
2022-05-22 & LoPeorDeEstasElecciones & Neutro & 357 \\
2022-05-22 & MiVotoEsPetroYFrancia & Izquierda & 2131 \\
2022-05-23 & MiVotoEsPetroYFrancia & Izquierda & 2131 \\
2022-05-23 & UnTramposoEs & Neutro & 1255 \\
2022-05-23 & FedericoEsColombia & Derecha & 1597 \\
2022-05-23 & MeInquieta & Neutro & 696 \\
2022-05-24 & ElDebateDefinitivo & Neutro & 7546 \\
2022-05-24 & AColombiaLePreocupa & Neutro & 1088 \\
2022-05-24 & LeApuestoA & Neutro & 326 \\
2022-05-24 & UnTramposoEs & Neutro & 1255 \\
2022-05-24 & GrandezaEs & Neutro & 498 \\
2022-05-25 & VotoPor & Neutro & 1093 \\
2022-05-25 & YaEsSuficiente & Izquierda & 816 \\
2022-05-25 & ElDebateDefinitivo & Neutro & 7546 \\
2022-05-25 & vanessapregúnteleafico & Izquierda & 323 \\
2022-05-25 & AColombiaLePreocupa & Neutro & 1088 \\
2022-05-25 & ConvenceUnoMásPorPetro & Izquierda & 174 \\
2022-05-26 & FicoElGanador & Derecha & 2578 \\
2022-05-26 & ElMejorCandidatoEs & Neutro & 1681 \\
2022-05-26 & ElDebateDecisivo & Neutro & 1305 \\
2022-05-26 & PetroEsElCambio & Izquierda & 457 \\
2022-05-26 & MagdalenaVotaPetro & Izquierda & 150 \\
2022-05-27 & PetroEs & Neutro & 877 \\
2022-05-27 & EsElMomentoDe & Neutro & 1334 \\
2022-05-27 & FicoElGanador & Derecha & 2578 \\
2022-05-27 & ElDomingoVoyA & Neutro & 298 \\
2022-05-27 & ElMejorCandidatoEs & Neutro & 1681 \\
2022-05-28 & LaVidaEnUnVoto & Izquierda & 221 \\
2022-05-28 & VoyConFico & Derecha & 78 \\
2022-05-28 & YoVotoPetroPresidente & Izquierda & 3376 \\
2022-05-28 & DebateFinal & Neutro & 5217 \\
2022-05-28 & VoyConFederico & Derecha & 4148 \\
2022-05-28 & FicoElGanador & Derecha & 2578 \\
2022-05-29 & EleccionesColombia & Neutro & 7088 \\
2022-05-29 & CualquieraMenosPetro & Derecha & 957 \\
2022-05-29 & Elecciones2022 & Neutro & 5978 \\
2022-05-29 & PetroPresidenteEnPrimera & Izquierda & 4032 \\
2022-05-29 & PetroPresidente2022 & Izquierda & 1712 \\
2022-05-29 & ElCambioEnPrimera & Izquierda & 3077 \\
2022-05-29 & SegundaVuelta & Neutro & 1752 \\
2022-05-29 & MiVotoEsSecretosky & Izquierda & 734 \\
2022-05-29 & VotoPorFicoYLara & Derecha & 846 \\
2022-05-29 & PetroNuncaSeráPresidente & Derecha & 461 \\
2022-05-29 & HoyMeIdentiFICO & Derecha & 92 \\
2022-05-29 & YoVotoPetroPresidente & Izquierda & 3376 \\
2022-05-29 & ColombiaConPetro & Izquierda & 3263 \\
2022-05-29 & VoyConFederico & Derecha & 4148 \\
2022-05-29 & ColombiaDecide & Neutro & 3906 \\
2022-05-29 & HoyGana & Neutro & 687 \\
2022-05-29 & PetroYFranciaSonElCambio & Izquierda & 637 \\
2022-05-29 & PetroNUNCAseraPresidente  & Derecha & 461 \\
2022-05-30 & SegundaVuelta & Neutro & 1752 \\
2022-05-30 & LaPrimeraVueltaFue & Neutro & 693 \\
2022-05-30 & Elecciones2022 & Neutro & 5978 \\
2022-05-30 & VotoPorFicoYLara & Derecha & 846 \\
2022-05-30 & HoyGana & Neutro & 687 \\
2022-05-31 & SegundaVuelta & Neutro & 1752 \\
2022-05-31 & MiCandidatoEs & Neutro & 2123 \\
2022-06-01 & FraudeElectoral & Izquierda & 2814 \\
2022-06-01 & VelezPregunteleAPetro & Derecha & 192 \\
2022-06-01 & pactosabroso & Izquierda & 79 \\
2022-06-01 & ElVerdaderoCambioEs & Neutro & 787 \\
2022-06-01 & RodolfoPresidente2022 & Derecha & 2720 \\
2022-06-01 & CreoEnColombiaPor & Neutro & 658 \\
2022-06-01 & Antipetrismo & Derecha & 176 \\
2022-06-02 & MeSumoA & Neutro & 307 \\
2022-06-02 & ColombiaNecesita & Neutro & 2381 \\
2022-06-02 & RodolfoPresidente2022 & Derecha & 2720 \\
2022-06-02 & UnaPreguntaParaPetroFm & Derecha & 850 \\
2022-06-02 & FraudeElectoral & Izquierda & 2814 \\
2022-06-02 & ElDebateFeminista & Izquierda & 56 \\
2022-06-03 & PetroElCambioSeguro & Izquierda & 3145 \\
2022-06-03 & RodolfoPresidente2022 & Derecha & 2720 \\
2022-06-03 & ColombiaQuiere & Neutro & 600 \\
2022-06-03 & ColombiaNecesita & Neutro & 2381 \\
2022-06-03 & UnDesastre & Neutro & 357 \\
2022-06-04 & PetroElCambioSeguro & Izquierda & 3145 \\
2022-06-04 & YoPactoConPetro & Izquierda & 761 \\
2022-06-04 & RodolfoPresidente2022 & Derecha & 2720 \\
2022-06-05 & LaCorrupcionPetrista & Derecha & 1492 \\
2022-06-05 & VotarEnBlancoEs & Neutro & 1466 \\
2022-06-05 & GraciasPero & Neutro & 719 \\
2022-06-05 & PetroElCambioSeguro & Izquierda & 3145 \\
2022-06-06 & VotarEnBlancoEs & Neutro & 1466 \\
2022-06-06 & MeLimpioELCuloConEsaLey & Izquierda & 149 \\
2022-06-06 & LaCorrupciónPetrista & Derecha & 775 \\
2022-06-06 & GraciasPero & Neutro & 719 \\
2022-06-06 & AliasElIngeniero & Izquierda & 505 \\
2022-06-07 & UnaVerdadEs & Neutro & 1504 \\
2022-06-07 & VotarEnBlancoEs & Neutro & 1466 \\
2022-06-08 & UnaBurlaEs & Neutro & 1467 \\
2022-06-08 & YoContratoAPetro & Izquierda & 1511 \\
2022-06-08 & NoQuiero & Neutro & 921 \\
2022-06-08 & UnaVerdadEs & Neutro & 1504 \\
2022-06-08 & ConPetroGanasTú & Izquierda & 259 \\
2022-06-09 & PetrismoSucio & Derecha & 5447 \\
2022-06-09 & RumboALaVictoria & Izquierda & 271 \\
2022-06-09 & PetroVideos & Derecha & 2011 \\
2022-06-09 & MeDaVergüenza & Neutro & 195 \\
2022-06-09 & PetroNoMateaRodolfo & Derecha & 37 \\
2022-06-09 & NoTodoVale & Neutro & 257 \\
2022-06-09 & PetroMentiroso & Derecha & 524 \\
2022-06-09 & LosPetroVideosSon & Derecha & 3034 \\
2022-06-09 & TodoVale & Neutro & 796 \\
2022-06-09 & YoContratoAPetro & Izquierda & 1511 \\
2022-06-09 & ColombiaEspera & Neutro & 918 \\
2022-06-10 & HablaMalDeColombia & Neutro & 2231 \\
2022-06-10 & PetrismoSucio & Derecha & 5447 \\
2022-06-10 & PetroVideos & Derecha & 2011 \\
2022-06-10 & CampañaSuciaEs & Neutro & 1149 \\
2022-06-10 & MeVoyConElIngeniero & Derecha & 278 \\
2022-06-11 & SoyPetroSoyPaz & Izquierda & 2125 \\
2022-06-11 & PetroVideos & Derecha & 2011 \\
2022-06-11 & HablaMalDeColombia & Neutro & 2231 \\
2022-06-11 & PetrismoSucio & Derecha & 5447 \\
2022-06-11 & QuéCansancio & Neutro & 459 \\
2022-06-12 & LaMaldadPetrista & Derecha & 2152 \\
2022-06-12 & SoyPetroSoyPaz & Izquierda & 2125 \\
2022-06-12 & ArizabaletaLameCulos & Izquierda & 328 \\
2022-06-13 & ArizabaletaSicarioMoral & Izquierda & 386 \\
2022-06-13 & PetroRespondaleAlosNiños & Derecha & 332 \\
2022-06-13 & VanessaEnSegundaVotoPor & Neutro & 199 \\
2022-06-13 & UnGolpeBajoEs & Neutro & 676 \\
2022-06-13 & EsUnaBajeza & Neutro & 501 \\
2022-06-13 & LaGranEncuesta & Neutro & 70 \\
2022-06-13 & LaMaldadPetrista & Derecha & 2152 \\
2022-06-13 & NosFalta & Neutro & 1155 \\
2022-06-14 & PetrismoAcosaALaPrensa & Derecha & 461 \\
2022-06-14 & YoBloqueoASemana & Izquierda & 3508 \\
2022-06-14 & LaCuotaDeBenedetti & Derecha & 416 \\
2022-06-14 & EstallidoSocialEs & Derecha & 1964 \\
2022-06-14 & NoMeDejaDormir & Neutro & 1178 \\
2022-06-15 & DebateObligadoEs & Neutro & 3491 \\
2022-06-15 & YoBloqueoASemana & Izquierda & 3508 \\
2022-06-15 & LoCorrectoEs & Neutro & 1495 \\
2022-06-15 & CaracolPetrista & Derecha & 409 \\
2022-06-15 & presidentepetro & Izquierda & 859 \\
2022-06-15 & EstallidoSocialEs & Derecha & 1964 \\
2022-06-16 & IrrespetuosoEs & Neutro & 2125 \\
2022-06-16 & debate & Neutro & 791 \\
2022-06-16 & NosHaceFalta & Neutro & 985 \\
2022-06-16 & RodolfoElPresidentedelPueblo & Derecha & 408 \\
2022-06-16 & MeDecepciona & Neutro & 452 \\
2022-06-17 & RHGanador & Derecha & 2277 \\
2022-06-17 & RodolfoCobarde & Izquierda & 4843 \\
2022-06-17 & YoVotoPor & Neutro & 1748 \\
2022-06-17 & EsteDomingo & Neutro & 1033 \\
2022-06-17 & PetroPresidenteEnsegunda & Izquierda & 1359 \\
2022-06-18 & ExguerrilleroOIngeniero & Neutro & 2760 \\
2022-06-18 & RegistraduriaResponda & Izquierda & 3107 \\
2022-06-18 & MiVotoEsAntiFraude & Izquierda & 1592 \\
2022-06-18 & RHGanador & Derecha & 2277 \\
2022-06-18 & PetroPresidenteEnsegunda & Izquierda & 1359 \\
2022-06-19 & PetroEsPresidente & Izquierda & 15521 \\
2022-06-19 & Elecciones2022 & Neutro & 5978 \\
2022-06-19 & EleccionesPresidenciales2022 & Neutro & 327 \\
2022-06-19 & ExguerrilleroOIngeniero & Neutro & 2760 \\
2022-06-19 & EleccionesColombia2022 & Neutro & 4484 \\
2022-06-19 & RegistraduriaResponda & Izquierda & 3107 \\
2022-06-19 & VivirSabroso & Izquierda & 790 \\
2022-06-20 & PetroEsPresidente & Izquierda & 15521 \\
2022-06-20 & ExguerrilleroOIngeniero & Neutro & 2760 \\
2022-06-20 & Elecciones2022 & Neutro & 5978 \\
2022-06-21 & PetroEsPresidente & Izquierda & 15521 \\
2022-06-21 & NuestraPrioridadEs & Neutro & 1253 \\
2022-06-21 & PetroBastaYa & Derecha & 564 \\
2022-06-21 & DePetroEspero & Neutro & 429 \\
2022-06-21 & PetroNecesita & Neutro & 377 \\
2022-06-22 & EsMuyImportante & Neutro & 1255 \\
2022-06-22 & PetroBastaYa & Derecha & 564 \\
2022-06-22 & LosImpuestosDePetro & Neutro & 359 \\
\end{longtable}


==> tables/tweets_ejemplos_1.tex <==
\begin{table}[!htbp]
\scriptsize
\begin{tabular}{{ | p{1.5cm}| p{11cm} | p{1.5cm} |}}
\hline
Numero de Ejemplo & Tweet & Orientacion política \\
\hline
1 & @lcvelez @lafm \#EstallidoSocialEs el arma de terror de Petro para obligar a votar por él. & Derecha \\
2 & Colombia va por el cambio, a redoblar esfuerzos estos 4 días para derrotar a la corrupción. \#PetroYFranciaSonElCambio \#EstallidoSocialEs & Derecha \\
3 & \#YaEsSuficiente Que los medios proclives al gbno, traten de darle aire boca a boca a un moribundo electoral, FICO. Ante su estancamiento en las encuestas y la distancia que le ha tomado Petro, pretenden en 1 acto de desesperacion, el insuflarlo de votantes de los cuales carece. & Izquierda \\
4 & \#YaEsSuficiente de mentir sobre @ingrodolfohdez , vayan a bucaramanga, vean lo que hizo y ahí si hablen.. & Izquierda \\
\hline
\end{tabular}
\caption{Ejemplos de tweets clasificados}
\label{table:ejemplos_1}
\end{table}


==> tables/tweets_ejemplos_2.tex <==
\begin{table}
\caption{Ejemplos de tweets clasificados}
\label{table:ejemplos_2}
\begin{tabular}{{ | p{2cm} | p{13cm} |}}
\toprule
Numero de Ejemplo & Tweet \\
\midrule
1 & \#AColombiaLePreocupa es la relación de @AndresPastrana\_ con la Unión Temporal Disproel, que es la que hace el conteo corrupto desde hace más de 20 años. ¿Pasos de animal grande sobre el control de las elecciones? \\
2 & \#TodoVale por eso es que estamos anclados al subdesarrollo, por anteponer todo por los principios. Un mentiroso y sucio Petro no le importa hacer lo que sea con tal de ganar. Los fines no justifican los medios. Petro acabó la posibilidad de un proyecto alternativo por su ego \\
3 & Juan Roberto Vargas es una persona decente. Néstor Morales es una porquería de persona. \#DebateFinal \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tweets_ejemplos_etiquetador.tex <==
\begin{table}[t]
\scriptsize
\begin{tabular}{{ | p{1.5cm}| p{7cm} | p{1.5cm} | p{1.5cm} | p{1.5cm} |}}
\hline
Numero de Ejemplo & Tweet & Etiquetador 1 & Etiquetador 2 & Etiquetador 3 \\
\hline
1 & \#LoPeorDeEstasElecciones es la división de la gente  de este país esta gente y cosas ya que pasan & Decepción & Decepción & Desagrado \\
2 & @Zuletalleras Son 4 años O es la. Derecha va realizar un golpe de estado? No cree a sus comentarios son ofensivos e incendiarios.... \#PetroEsPresidente & Miedo, Incertidumbre & Miedo & Asco, Desagrado \\
\hline
\end{tabular}
\caption{Ejemplos de tweets clasificados por etiquetador}
\label{table:ejemplos_etiquetador}
\end{table}


==> tables/tweets_ejemplos_multiples.tex <==
\begin{table}[!htbp]
\scriptsize
\begin{tabular}{{| p{1.5cm} | p{11.5cm} | p{1cm} |}}
\hline
Numero de Ejemplo & Tweet & Etiquetas \\
\hline
1 & En \#ElDebateDefinitivo Fajardo con sus preguntas hizo subir de votos a @petrogustavo en los votos de los indecisos. La ausencia del ingeniero ayudó a Petro, Fico pierde sólo. \#PetroGanaDebate, es el único candidato que gana con argumentos. & alegria, asco \\
2 & Comenzo el entrampamiento público en el debate presidencial. Ya ni disimulan. \#ElDebateDefinitivo & tristeza, asco \\
3 & Fajardo quedo tan peinado que ya se quiere ir \#ElDebateDefinitivo & tristeza, asco \\
4 & En conclusión \#ElDebateDefinitivo deja claro que Petro es un peligro. Mentiroso, arrogante, tramposo, encubridor, manipulador, violento, pasivo agresivo, resentido. En resumen, una porquería de ser humano, qué digo humano... un demonio.  Petro es el Pol Pot de Ciénaga de Oro & miedo, asco \\
\hline
\end{tabular}
\caption{Ejemplos de tweets con etiquetas múltiples}
\label{table:ejemplos_multples}
\end{table}


==> tables/tweets_ejemplos_preds.tex <==
\begin{table}[!htbp]
\scriptsize
\begin{tabular}{{ | p{1.5cm} | p{9cm} | p{1.5cm} | p{1.5cm} | }}
\hline
Numero de Ejemplo & Tweet & Etiquetas & Predicciones \\
\hline
1 & En conclusión \#ElDebateDefinitivo deja claro que Petro es un peligro. Mentiroso, arrogante, tramposo, encubridor, manipulador, violento, pasivo agresivo, resentido. En resumen, una porquería de ser humano, qué digo humano... un demonio.  Petro es el Pol Pot de Ciénaga de Oro & Miedo, Asco & Asco \\
2 & \#ElDebateDefinitivo @sergio\_fajardo  fue a vender ilusiones y convencer no a debatir no propone sólo dice redundancias, me sorprende profe sera que de proyectos no sabe tanto como de licenciatura... & Tristeza, Asco & Asco \\
3 & Juan Roberto Vargas es una persona decente. Néstor Morales es una porquería de persona. \#DebateFinal & Alegria, Asco & Asco \\
4 & \#FedericoEsColombia Me uno Federico Gutiérrez es Colombia. & Neutral & Alegria \\
\hline
\end{tabular}
\caption{Ejemplos de tweets con divergencias entre etiquetas y clasificaciones}
\label{table:ejemplos_preds}
\end{table}


==> tables/tweets_ejemplos_test.tex <==
\begin{table}
\caption{Ejemplos de tweets clasificados}
\label{table:ejemplos_test}
\begin{tabular}{{ | p{13cm} | p{2cm} |}}
\toprule
Tweet & Orientacion política \\
\midrule
@lcvelez @lafm \#EstallidoSocialEs el arma de terror de Petro para obligar a votar por él. & Derecha \\
Colombia va por el cambio, a redoblar esfuerzos estos 4 días para derrotar a la corrupción. \#PetroYFranciaSonElCambio \#EstallidoSocialEs & Derecha \\
\#YaEsSuficiente Que los medios proclives al gbno, traten de darle aire boca a boca a un moribundo electoral, FICO. Ante su estancamiento en las encuestas y la distancia que le ha tomado Petro, pretenden en 1 acto de desesperacion, el insuflarlo de votantes de los cuales carece. & Izquierda \\
\#YaEsSuficiente de mentir sobre @ingrodolfohdez , vayan a bucaramanga, vean lo que hizo y ahí si hablen.. & Izquierda \\
\#LoPeorDeEstasElecciones es la división de la gente  de este país esta gente y cosas ya que pasan & Neutro \\
@Zuletalleras Son 4 años
O es la. Derecha va realizar un golpe de estado?
No cree a sus comentarios son ofensivos e incendiarios....
\#PetroEsPresidente & Izquierda \\
\bottomrule
\end{tabular}
\end{table}

